Physical Operating-Condition-Guided Vision-Language Matching for Cavitation Diagnosis in Industrial Pipeline Systems

Cavitation diagnosis in industrial pipeline systems is challenging because acoustic responses vary substantially with operating conditions, while similar time-frequency patterns may correspond to different cavitation states. To address this issue, we propose a physical operating-condition-guided vision-language matching (POC-VLM) for cavitation diagnosis. POC-VLM first constructs physical operating-condition-aware semantic descriptions by explicitly incorporating sample-specific operating variables into candidate cavitation texts. A time-frequency-conditioned text adaptation module then dynamically aligns these physical semantics with the observed acoustic response, followed by global-local vision-language matching to capture both holistic and localized discriminative patterns. In parallel, a K-nearest neighbours-based non-parametric physical operating-condition prior estimates the physical plausibility of each candidate state and is fused with the vision-language semantic evidence at the decision level. Experiments on three real-world cavitation datasets show that POC-VLM consistently outperforms representative data-driven, multimodal and domain-specific diagnostic methods. Further analyses verify the complementary roles of vision-language semantic matching and physical operating-condition priors, while demonstrating robust performance under varying sampling rates, noise levels and observation durations.

==> input_figs/input_PressureFlowModel.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.6\textwidth,height=45mm]{figs/app/pressure_flow_model.pdf}
    \caption{Pressure flow model in a valve. The solid black, dotted orange, dotted green and dotted blue lines are represented by the upstream pressure $p_u$, the downstream pressure $p_d$, the minimum pressure $p_{\min}$ and the vapor pressure $p_v$, respectively.}
    \label{fig: civitation knowledge}
\end{figure}

